You Never Get a Second Chance To Make a Good First Impression: Seeding Active Learning for 3D Semantic Segmentation

We propose SeedAL, a method to seed active learning for efficient annotation of 3D point clouds for semantic segmentation. Active Learning (AL) iteratively selects relevant data fractions to annotate within a given budget, but requires a first fraction of the dataset (a 'seed') to be already annotated to estimate the benefit of annotating other data fractions. We first show that the choice of the seed can significantly affect the performance of many AL methods. We then propose a method for automatically constructing a seed that will ensure good performance for AL. Assuming that images of the point clouds are available, which is common, our method relies on powerful unsupervised image features to measure the diversity of the point clouds. It selects the point clouds for the seed by optimizing the diversity under an annotation budget, which can be done by solving a linear optimization problem. Our experiments demonstrate the effectiveness of our approach compared to random seeding and existing methods on both the S3DIS and SemanticKitti datasets. Code is available at https://github.com/nerminsamet/seedal.

==> data/s3dis/s3dis_coreset_random-mean.tex <==
x y
3 30.1
5 33.6
7 36.2
9 37.5

==> data/s3dis/s3dis_coreset_random-mean2.tex <==
x y
3 30.1
5 33.6
7 36.2
9 37.5

==> figs/tikz/table_kitti.tex <==
\centering
    \begin{tabular}{c|c|cccccccc} %
        \bfseries cycle & initial set & \random & \softconf &  \softentropy & \softmargin & \coreset & \mcdropout & \segent & \redal \\  % specify table head
        \toprule
        \csvreader[head to column names]{data/kitti/new/all_rest_kitt_c1.csv}{}% use head of csv as column names
        {\\ 1 & random & 
        \randomrandom 	$\pm$ \randomrandomstd  & \softmaxconfidencerandom $\pm$ \softmaxconfidencerandomstd 
        & \softmaxentropyrandom $\pm$ \softmaxentropyrandomstd
        & \softmaxmarginrandom  $\pm$ \softmaxmarginrandomstd
        & \coresetrandom $\pm$ \coresetrandomstd
        & \mcdropoutrandom $\pm$ \mcdropoutrandomstd 
        & \segmententropyrandom  $\pm$ \segmententropyrandomstd
        & \ReDALrandom $\pm$ \ReDALrandomstd}
        
        \csvreader[head to column names]{data/kitti/new/all_rest_kitt_c1.csv}{}% use head of csv as column names
        {\\ 1 & Rseed & \randomredal  & \softmaxconfidenceredal  & \softmaxentropyredal  & \softmaxmarginredal  & \coresetredal & \mcdropoutredal & \segmententropyredal  & \ReDALredal}
        % \\        
        \csvreader[head to column names]{data/kitti/new/all_rest_kitt_c1.csv}{}% use head of csv as column names
        {\\ 1 & \KMfirst & \randomkmvone  & \softmaxconfidencekmvone  & \softmaxentropykmvone  & \softmaxmarginkmvone  & \coresetkmvone & \mcdropoutkmvone & \segmententropykmvone  & \ReDALkmvone}
        
        \csvreader[head to column names]{data/kitti/new/all_rest_kitt_c1.csv}{}% use head of csv as column names
        {\\ 1 & \KMsecond & \randomkmvtwo  & \softmaxconfidencekmvtwo  & \softmaxentropykmvtwo  & \softmaxmarginkmvtwo  & \coresetkmvtwo & \mcdropoutkmvtwo & \segmententropykmvtwo  & \ReDALkmvtwo}
        
        \csvreader[head to column names]{data/kitti/new/all_rest_kitt_c1.csv}{}% 
        {\\ 1 & \ours & \randomfullmethod &  \softmaxconfidencefullmethod  &  \softmaxentropyfullmethod  &  \softmaxmarginfullmethod  &  \coresetfullmethod &  \mcdropoutfullmethod &  \segmententropyfullmethod  &  \ReDALfullmethod}
        \\\midrule

       \csvreader[head to column names]{data/kitti/new/all_rest_kitt_c2.csv}{}% use head of csv as column names
        {\\ 2 & random & \randomredal  & \softmaxconfidenceredal  & \softmaxentropyredal  & \softmaxmarginredal  & \coresetredal & \mcdropoutredal & \segmententropyredal  &  \ReDALredal}
        % \\
        \csvreader[head to column names]{data/kitti/new/all_rest_kitt_c2.csv}{}% use head of csv as column names
        {\\ 2 & \KMfirst & \randomkmvone  & \softmaxconfidencekmvone  & \softmaxentropykmvone  & \softmaxmarginkmvone  & \coresetkmvone & \mcdropoutkmvone & \segmententropykmvone  & \ReDALkmvone}
        \csvreader[head to column names]{data/kitti/new/all_rest_kitt_c2.csv}{}% use head of csv as column names
        {\\ 2 & \KMsecond & \randomkmvtwo  & \softmaxconfidencekmvtwo  & \softmaxentropykmvtwo  & \softmaxmarginkmvtwo  & \coresetkmvtwo & \mcdropoutkmvtwo & \segmententropykmvtwo  & \ReDALkmvtwo}
        \csvreader[head to column names]{data/kitti/new/all_rest_kitt_c2.csv}{}% use head of csv as column names
        {\\ 2 & \ours &  \randomfullmethod  &  \softmaxconfidencefullmethod  &  \softmaxentropyfullmethod  &  \softmaxmarginfullmethod  &  \coresetfullmethod &  \mcdropoutfullmethod &  \segmententropyfullmethod  &  \ReDALfullmethod}
        \\\midrule

        \csvreader[head to column names]{data/kitti/new/all_rest_kitt_c3.csv}{}% use head of csv as column names
        {\\ 3 & random & \randomredal  & \softmaxconfidenceredal  & \softmaxentropyredal  & \softmaxmarginredal  & \coresetredal & \mcdropoutredal & \segmententropyredal  &  \ReDALredal}
        % \\
        \csvreader[head to column names]{data/kitti/new/all_rest_kitt_c3.csv}{}% use head of csv as column names
        {\\ 3 & \KMfirst & \randomkmvone  & \softmaxconfidencekmvone  & \softmaxentropykmvone  & \softmaxmarginkmvone  & \coresetkmvone & \mcdropoutkmvone & \segmententropykmvone  & \ReDALkmvone}
        \csvreader[head to column names]{data/kitti/new/all_rest_kitt_c3.csv}{}% use head of csv as column names
        {\\ 3 & \KMsecond & \randomkmvtwo  & \softmaxconfidencekmvtwo  & \softmaxentropykmvtwo  & \softmaxmarginkmvtwo  & \coresetkmvtwo & \mcdropoutkmvtwo & \segmententropykmvtwo  & \ReDALkmvtwo}
        \csvreader[head to column names]{data/kitti/new/all_rest_kitt_c3.csv}{}% use head of csv as column names
        {\\ 3 & \ours &  \randomfullmethod  &  \softmaxconfidencefullmethod  &  \softmaxentropyfullmethod  &  \softmaxmarginfullmethod  &  \coresetfullmethod &  \mcdropoutfullmethod &  \segmententropyfullmethod  & \ReDALfullmethod}
        \\\midrule
       
       \csvreader[head to column names]{data/kitti/new/all_rest_kitt_c4.csv}{}% use head of csv as column names
        {\\ 4 & random & \randomredal  & \softmaxconfidenceredal  & \softmaxentropyredal  & \softmaxmarginredal  & \coresetredal & \mcdropoutredal & \segmententropyredal  & \ReDALredal}
        % \\
        \csvreader[head to column names]{data/kitti/new/all_rest_kitt_c4.csv}{}% use head of csv as column names
        {\\ 4 & \KMsecond & \randomkmvtwo  & \softmaxconfidencekmvtwo  & \softmaxentropykmvtwo  & \softmaxmarginkmvtwo  & \coresetkmvtwo & \mcdropoutkmvtwo & \segmententropykmvtwo  & \ReDALkmvtwo}
        \csvreader[head to column names]{data/kitti/new/all_rest_kitt_c4.csv}{}% use head of csv as column names
        {\\ 4 & \ours &  \randomfullmethod  &  \softmaxconfidencefullmethod  &  \softmaxentropyfullmethod  &  \softmaxmarginfullmethod  & \coresetfullmethod &  \mcdropoutfullmethod &  \segmententropyfullmethod  &  \ReDALfullmethod}
        \\\midrule

    \end{tabular}

==> pgfplotstableset_s3dis.tex <==
\pgfplotstableset{
    create on use/Ymd15/.style={create col/copy column from table={data/s3dis/s3dis_mc_dropout_init_set_15_closest_dino.txt}{y}}
}

\pgfplotstableset{
    create on use/Yredal15/.style={create col/copy column from table={data/s3dis/s3dis_ReDAL_init_set_15_closest_dino.txt}{y}}
}

\pgfplotstableset{
    create on use/Yrand15/.style={create col/copy column from table={data/s3dis/s3dis_random_init_set_15_closest_dino.txt}{y}}
}

\pgfplotstableset{
    create on use/Ysege15/.style={create col/copy column from table={data/s3dis/s3dis_segment_entropy_init_set_15_closest_dino.txt}{y}}
}

\pgfplotstableset{
    create on use/Ysofc15/.style={create col/copy column from table={data/s3dis/s3dis_softmax_confidence_init_set_15_closest_dino.txt}{y}}
}

\pgfplotstableset{
    create on use/Ycs10/.style={create col/copy column from table={data/s3dis/s3dis_coreset_init_set_10_closest_dino.txt}{y}}
}

\pgfplotstableset{
    create on use/Yredal10/.style={create col/copy column from table={data/s3dis/s3dis_ReDAL_init_set_10_closest_dino.txt}{y}}
}

\pgfplotstableset{
    create on use/Ysege10/.style={create col/copy column from table={data/s3dis/s3dis_segment_entropy_init_set_10_closest_dino.txt}{y}}
}

\pgfplotstableset{
    create on use/Ysofc10/.style={create col/copy column from table={data/s3dis/s3dis_softmax_confidence_init_set_10_closest_dino.txt}{y}}
}

\pgfplotstableset{
    create on use/Ysofe10/.style={create col/copy column from table={data/s3dis/s3dis_softmax_entropy_init_set_10_closest_dino.txt}{y}}
}

\pgfplotstableset{
    create on use/Ysofm10/.style={create col/copy column from table={data/s3dis/s3dis_softmax_margin_init_set_10_closest_dino.txt}{y}}
}

\pgfplotstableset{
    create on use/Yredal/.style={create col/copy column from table={data/s3dis/s3dis_ReDAL_init_set_6_closest_dino.txt}{y}}
}
\pgfplotstableset{
    create on use/Yrandom/.style={create col/copy column from table={data/s3dis/s3dis_random_init_set_6_closest_dino.txt}{y}}
}
\pgfplotstableset{
    create on use/Ycs/.style={create col/copy column from table={data/s3dis/s3dis_coreset_init_set_6_closest_dino.txt}{y}}
}
\pgfplotstableset{
    create on use/Ymc/.style={create col/copy column from table={data/s3dis/s3dis_mc_dropout_init_set_6_closest_dino.txt}{y}}
}
\pgfplotstableset{
    create on use/Yse/.style={create col/copy column from table={data/s3dis/s3dis_segment_entropy_init_set_6_closest_dino.txt}{y}}
}
\pgfplotstableset{
    create on use/Ysoc/.style={create col/copy column from table={data/s3dis/s3dis_softmax_confidence_init_set_6_closest_dino.txt}{y}}
}
\pgfplotstableset{
    create on use/Ysoe/.style={create col/copy column from table={data/s3dis/s3dis_softmax_entropy_init_set_6_closest_dino.txt}{y}}
}
\pgfplotstableset{
    create on use/Ysom/.style={create col/copy column from table={data/s3dis/s3dis_softmax_margin_init_set_6_closest_dino.txt}{y}}
}
